Montessori-Instruct: Generate Influential Training Data Tailored for Student Learning

Synthetic data has been widely used to train large language models, but their generative nature inevitably introduces noisy, non-informative, and misleading learning signals. In this paper, we propose Montessori-Instruct, a novel data synthesis framework that tailors the data synthesis ability of the teacher language model toward the student language model's learning process. Specifically, we utilize local data influence of synthetic training data points on students to characterize students' learning preferences. Then, we train the teacher model with Direct Preference Optimization (DPO) to generate synthetic data tailored toward student learning preferences. Experiments with Llama3-8B-Instruct (teacher) and Llama3-8B (student) on Alpaca Eval and MT-Bench demonstrate that Montessori-Instruct significantly outperforms standard synthesis methods by 18.35\% and 46.24\% relatively. Our method also beats data synthesized by a stronger teacher model, GPT-4o. Further analysis confirms the benefits of teacher's learning to generate more influential training data in the student's improved learning, the advantages of local data influence in accurately measuring student preferences, and the robustness of Montessori-Instruct across different student models. Our code and data are open-sourced at https://github.com/cxcscmu/Montessori-Instruct.

==> tables/analysis/abl_on_iterations.tex <==
\begin{table}[h]
\caption{Ablation studies on seed data}
    \centering
    \scalebox{0.9}{
        \begin{tabular}{lccc}
        \toprule
        \multirow{2}{*}{Seed dataset}&
          \multicolumn{2}{l}{Alpaca Eval 2.0} &
          MT-Bench \\
          \cmidrule(lr){2-3} \cmidrule(lr){4-4} 
                    & LC-WR & WR & Score \\
        \rowcolor{blue!5}
        \midrule
        iter-1\_2000 &       52.28\%&    54.76\%&         6.715\\
        \midrule
        \midrule
        \rowcolor{blue!10}
        iter-2\_2000 &       53.48\%&    56.82\%&         6.807\\
        \textit{( iter-1} &  \textit{54.92}\% &  \textit{58.59\%} & \textit{6.825 )}\\  
        \midrule
        \midrule
        \rowcolor{blue!15}
        iter-3\_2000 &  55.25\%&    58.47\%&    6.962\\  \textit{( iter-2} &  \textit{56.37\%} &  \textit{60.15\%} & \textit{7.163 )} \\  
        \bottomrule
        \end{tabular}
    }
\label{tab:abl_on_iterations}
\end{table}

==> tables/analysis/abl_on_reward.tex <==
\begin{table}[t]
\vspace{5mm}
\caption{Ablation Studies on how to evaluate the influence of each data point. All experiments were conducted using the 8B teacher and 8B student models.}
    \centering
    \resizebox{1.0\textwidth}{!}{
        \begin{tabular}{lcccccccc}
        \toprule
        \multirow{2}{*}{Methods}&
          \multicolumn{2}{l}{Alpaca Eval 2.0} &
          MT-Bench &
          \multirow{1}{*}{MMLU} &
          \multirow{1}{*}{GPQA}&
          \multirow{1}{*}{ARC-C}&
          \multirow{1}{*}{GSM8K}&
          \multirow{1}{*}{HellaSwag} \\
          \cmidrule(lr){2-3}
          \cmidrule(lr){4-4}
          \cmidrule(lr){5-9}
                    & LC-WR & WR & Score &  \multicolumn{5}{c}{Accuracy}  \\
        \midrule
        % \rowcolor{blue!10}
        LLM-as-a-Judge &       53.42\%&    54.93\%&         6.731&  62.93&  29.75&  62.09&  58.82&  81.05\\
        % \rowcolor{blue!5}
        Training loss &       52.34\%&    54.99\%&         6.656&  62.54&  29.89&  61.48&  58.76& 80.93\\
        % \rowcolor{blue!15}
        Local data influence&  54.92\%&    58.59\%&    6.825&  62.93&  29.91&  62.97&  58.76&  81.22\\    
        \bottomrule
        \end{tabular}
    }
\label{tab:abl_on_reward}
\end{table}

==> tables/analysis/abl_on_seed_data.tex <==
\begin{table}[t]
\caption{Ablation studies on the seed data used in Montessori-Instruct. OOD denotes the \textbf{O}ut-\textbf{O}f-\textbf{D}omain seed, ID refers to the \textbf{I}n-\textbf{D}omain seed, and Test indicates the direct use of the \textbf{test set} as the seed.}
    \centering
    \resizebox{1.0\textwidth}{!}{
        \begin{tabular}{lcccccccc}
        \toprule
        \multirow{2}{*}{Seed data}&
          \multicolumn{2}{l}{Alpaca Eval 2.0} &
          MT-Bench &
          \multirow{1}{*}{MMLU} &
          \multirow{1}{*}{GPQA}&
          \multirow{1}{*}{ARC-C}&
          \multirow{1}{*}{GSM8K}&
          \multirow{1}{*}{HellaSwag} \\
          \cmidrule(lr){2-3}
          \cmidrule(lr){4-4}
          \cmidrule(lr){5-9}
                    & LC-WR & WR & Score &  \multicolumn{5}{c}{Accuracy}  \\
        \midrule
        \rowcolor{blue!5}
        Open Assistant (OOD) &       52.28\%&    54.76\%&         6.706&  62.86&  29.74&  62.29&  58.42&  81.24\\
        \rowcolor{blue!10}
        Alpaca GPT4 (ID) &       54.92\%&    58.59\%&         6.825&  62.93&  29.91&  62.97&  58.76& 81.22\\
        \rowcolor{blue!15}
        Alpaca Eval (Test) &  57.64\%&    61.36\%&    7.147&  62.93&  30.44&  63.06&  60.80&  81.09\\    
        \bottomrule
        \end{tabular}
    }
\label{tab:abl_on_seed}
\end{table}

==> tables/analysis/abl_on_teacher_and_responses.tex <==
\begin{table}[t]
\caption{Ablation studies on two optimization objects in Montessori-Instruct: \textbf{responses} optimization based on instructions and \textbf{teacher models} optimization.}
    \centering
    \resizebox{1.0\textwidth}{!}{
        \begin{tabular}{lcccccccc}
        \toprule
        \multirow{2}{*}{Methods} &
          \multicolumn{2}{l}{Alpaca Eval 2.0} &
          MT-Bench &
          \multirow{1}{*}{MMLU} &
          \multirow{1}{*}{GPQA}&
          \multirow{1}{*}{ARC-C}&
          \multirow{1}{*}{GSM8K}&
          \multirow{1}{*}{HellaSwag} \\
          \cmidrule(lr){2-3}
          \cmidrule(lr){4-4}
          \cmidrule(lr){5-9}
                    & LC-WR & WR & Score &  \multicolumn{5}{c}{Accuracy}  \\
        \midrule
        Self-Instruct &       50\%&    50\%&         6.490&  62.42&  31.92&  59.98&  58.76&  80.93\\
        % \rowcolor{red!5}
        Bootstrap &       50.59\%&    48.14\%&         6.618&  60.67&  25.19&  57.95&  58.13&  80.46\\
        % \rowcolor{red!5}
        Response optimization    &       51.59\%&    54.22\%&    6.556&  62.43&  27.45&  60.42&  56.38&  81.04\\    
        % \rowcolor{blue!5}
        Montessori-Instruct &       54.92\%&    58.59\%&         6.825&  62.93&  29.91&  62.97&  58.76& 81.22\\
        \bottomrule
        \end{tabular}
    }
\label{tab:abl_on_teacher_and_responses}
\end{table}

==> tables/archive/1B_result.tex <==

\begin{table}[t]
  \centering
    \scalebox{0.9}{
        \begin{tabular}{lccc}
        \toprule
        \multirow{2}{*}{ } & \multicolumn{2}{c}{Alpaca Eval 2.0} & \multicolumn{1}{c}{MT-Bench} \\
        \cmidrule(lr){2-3} \cmidrule(lr){4-4}
         Methods & LC-WR & WR & Overall \\

        \midrule
        pertrained model  & 17.89\% & 17.56 \% & 1.02 \\
        \midrule
        \textbf{\textit{Self-Instruct}} & & & \\
        Llama3-8B-Instruct$_{\: teacher}$\zichun{Teacher=...} & 50\%& 50\%& 2.154\\
        gpt-4o$_{\: teacher}$ \zichun{Teacher=...} & 54.02\%& 55.02\%& 1.928\\
        \midrule
        
        \textbf{\textit{Self-reward}} & & & \\
        % base model + \textbf{iter 1} & 4500(dpo)& 13.13\%& 14.08\%& 3.712\\
        % base model + \textbf{iter 2} & - & - & - & -\\
        iter 1 & - & - & - \\
        iter 2 & - & - & - \\
        
        \midrule
        \textbf{\textit{LLM2LLM}} & & & \\
        iter 1 & 52.03\%& 52.75\%& 2.243\\
        iter 2 & 51.64\%& 53.52\%& 2.192\\
        % base model + \textbf{iter 1} & 10872& 42.15\%& 41.79\%& 5.778\\
        % base model + \textbf{iter 2} & - & - & - & -\\

        \midrule
        \textbf{\textit{Ours}} & & & \\
        iter 1 & 53.25\% & 51.77\%  & 2.485\\
        iter 2 & 54.37\% & 54.68\% & 2.526\\
        
        \bottomrule
        \end{tabular}
    }
\caption{Results for 1B model}
\label{tab:1B-result}
\end{table}

==> tables/archive/main_results.tex <==

\begin{table}[t]
  \centering
    \scalebox{0.9}{
        \begin{tabular}{lcccccc}
        \toprule
        \multirow{2}{*}{ } & \multicolumn{3}{c}{LLama3-8B$_{\: student}$} & \multicolumn{3}{c}{TinyLLama-1.1B$_{\: student}$} \\
        \cmidrule(lr){2-4} \cmidrule(lr){5-7}
        & \multicolumn{2}{c}{Alpaca Eval 2.0} & \multicolumn{1}{c}{MT-Bench} & \multicolumn{2}{c}{Alpaca Eval 2.0} & \multicolumn{1}{c}{MT-Bench} \\
        \cmidrule(lr){2-3} \cmidrule(lr){4-4} \cmidrule(lr){5-6} \cmidrule(lr){7-7}
         Methods & LC-WR & WR & Overall & LC-WR & WR & Overall \\

        \midrule
        pertrained model  & 2.09\% & 3.39\% & 5.597& 17.89\% & 17.56 \% & 1.02 \\
        \midrule
        \textbf{\textit{Self-Instruct}} & & & & & & \\
        Llama3-8B-Instruct$_{\: teacher}$ & 50\%& 50\%& 6.490 & 50\%& 50\%& 2.154\\
        gpt-4o$_{\: teacher}$ & 54.95\%& 56.39\%& 5.918& 54.02\%& 55.02\%& 1.928\\
        \midrule
        
        \textbf{\textit{Self-reward}} & & & & & & \\
        % base model + \textbf{iter 1} & 4500(dpo)& 13.13\%& 14.08\%& 3.712\\
        % base model + \textbf{iter 2} & - & - & - & -\\
        iter 1 & - & - & - & - & - & - \\
        iter 2 & - & - & - & - & - & - \\
        
        \midrule
        \textbf{\textit{LLM2LLM}} & & & & & & \\
        iter 1 & 51.49\%& 53.12\%& 6.531& 52.03\%& 52.75\%& 2.243\\
        iter 2 & 52.63\%& 55.02\%& 6.519& 51.64\%& 53.52\%& 2.192\\
        % base model + \textbf{iter 1} & 10872& 42.15\%& 41.79\%& 5.778\\
        % base model + \textbf{iter 2} & - & - & - & -\\

        \midrule
        \textbf{\textit{Ours}} & & & & & & \\
        iter 1 & 54.92\%& 58.59\%& 6.825 & 53.25\% & 51.77\%  & 2.485\\
        iter 2 & \textbf{56.37}\% & \textbf{60.15}\%& \textbf{7.148} & 54.37\% & 54.68\% & 2.526\\
        
        \bottomrule
        \end{tabular}
    }
\caption{Main Results}
\label{tab:main-result}
\vspace{-5mm} 
\end{table}

==> tables/archive/nlp_benchmarks.tex <==

\begin{table}[h]
  \centering
    \scalebox{0.74}{
        \begin{tabular}{lccccc}
        \toprule
        Models & MMLU & ARC-E & ARC-C & GSM8K & HellaSwag \\
        \midrule
        pretrained model & 62.68& 60.82& 38.57& 47.01& 58.64\\
        \midrule
        \textbf{\textit{Self-Instruct}} & & & & & \\
        Llama3-8B-Instruct$_{\: teacher}$ & 65.42& 74.24& 46.42& 48.12& 59.58\\
        gpt-4o$_{\: teacher}$ & 69.41& 78.87& 50.51& 48.75& 58.2\\

        \midrule
        \textbf{\textit{Self-reward}} & & & & & \\
        iter 1 & - & - & - & - & -\\
            iter 2 & - & - & - & - & -\\
        
        \midrule
       \textbf{ \textit{LLM2LLM}} & & & & &\\
        iter 1 & - & 76.12& 47.49& 47.28& 56.47\\
        iter 2 & - & 77.04& 49.65& 48.75& 54.68\\

        \midrule
        \textit{\textbf{Ours}} & & & & &\\
        iter 1 & 68.93& 76.56& 48.21& 51.02& 59.03\\
        iter 2 & 69.47& 79.12& 51.62& 58.15& 59.04\\
        
        \bottomrule
        \end{tabular}
    }
\caption{General NLP Benchmarks \cx{merge with table 3?} \xiaochuan{I am worried that the line width may not be enough to merge this table with the main table. Since all results of table 3 are based on the 8B model, one approach is to only place the 8B results and those of table3 in the main table, while placing the result of 1B separately.} \cx{1B can go to appendix}}
% \vspace{-5mm} 
\label{tab:nlp-benchmarks}
\end{table}

